Towards Interpretable Protein Structure Prediction with Sparse Autoencoders

Protein language models have revolutionized structure prediction, but their nonlinear nature obscures how sequence representations inform structure prediction. While sparse autoencoders (SAEs) offer a path to interpretability here by learning linear representations in high-dimensional space, their application has been limited to smaller protein language models unable to perform structure prediction. In this work, we make two key advances: (1) we scale SAEs to ESM2-3B, the base model for ESMFold, enabling mechanistic interpretability of protein structure prediction for the first time, and (2) we adapt Matryoshka SAEs for protein language models, which learn hierarchically organized features by forcing nested groups of latents to reconstruct inputs independently. We demonstrate that our Matryoshka SAEs achieve comparable or better performance than standard architectures. Through comprehensive evaluations, we show that SAEs trained on ESM2-3B significantly outperform those trained on smaller models for both biological concept discovery and contact map prediction. Finally, we present an initial case study demonstrating how our approach enables targeted steering of ESMFold predictions, increasing structure solvent accessibility while fixing the input sequence. To facilitate further investigation by the broader community, we open-source our code, dataset, pretrained models https://github.com/johnyang101/reticular-sae , and visualizer https://sae.reticular.ai .

==> discussion/v1.tex <==
In this work, we trained sparse autoencoders with different architectures to extract interpretable features from ESM2, building on recent work using SAEs to understand protein language models (\cite{Simon2024.11.14.623630}; \cite{Adams2025.02.06.636901}). By scaling SAE training to ESM2-3B for the first time and demonstrating targeted interventions on ESMFold's structure predictions through feature steering, we provide new perspectives on how model capabilities and interpretability scale with model size, and how SAE features can influence both sequence and structural properties in protein models.

Our results demonstrate that larger language models capture substantially more biological concepts in superposition, with ESM2-3B encoding nearly 3x more interpretable features than ESM2-8M. The hierarchical organization enabled by Matryoshka SAEs allows us to effectively compress and manipulate these representations while maintaining model performance.

==> discussion/v3.tex <==
This work advances PLM interpretability by scaling SAEs to ESM2-3B, extending recent work using SAEs to interpret PLMs to the structure prediction task (\cite{Simon2024.11.14.623630}; \cite{Adams2025.02.06.636901}). Through a combination of increasing subject model size, leveraging the Matryoshka architecture, and targeted interventions on ESMFold's structure predictions, we present the first work applying mechanistic interpretability to protein structure prediction.

\subsection{Limitations}

In the scope of this work, several limitations remain. First, although we take an important step toward mechanistic interpretability of protein structure prediction, our focus is exclusively on how PLM-derived sequence representations inform structure prediction. The interpretability of ESMFold's structure prediction head is left for future investigation. Second, our interventions on ESMFold were restricted to single-feature manipulations on embeddings from individual layers rather than exploring combinations of features or cross-layer interactions. Third, our analysis is limited to the 8M and 3B models of ESM2; evaluating a broader range of model sizes could reveal whether SAE performance eventually plateaus. Fourth, ESMFold is no longer state-of-the-art compared to newer diffusion-based protein structure prediction methods  \cite{Abramson2024, WohlwendBoltz124, Watson2023}. 

Fifth, recent work suggests that SAEs can learn different features even when trained on the same data, implying that our results may be sensitive to both initialization and the specific UniRef50 sample used (\cite{paulo2025sparseautoencoderstraineddata}). Sixth, our structural steering experiments focused primarily on surface accessibility, leaving other potential structural properties unexplored, and the observed hydrophobicity effects might be achievable through simpler approaches such as steering smaller PLMs or using supervised linear probes. Seventh, for Matryoshka SAEs, we do not report how the number of groups and group size choices impact results. Finally, although our ablation studies demonstrate preservation of structural information, we have not fully characterized how interactions among SAE features might affect ESMFold’s folding mechanism. We anticipate that future work leveraging our open-source models developed with substantial computational resources will address these limitations and yield further insights for the community.

% In the scope of this work, several limitations remain:
% First, while taking a significant step towards mechanistic interpretability of protein structure prediction, this work focuses only on how PLM learned sequence representations inform structure prediction, leaving interpretability of the structure prediction head to future work. Second, our interventions on ESMFold were limited to manipulating single features and only on embeddings from individual layers, rather than exploring combinations of features or cross-layer interactions. We hope that future work will build on our open-source models which took considerable resources to train and 

% our analysis focuses only on ESM2-8M and 3B; studying a broader range of model sizes could reveal whether SAE performance eventually plateaus. Second, ESMFold is no longer state-of-the-art compared to diffusion-based protein structure prediction methods \cite{Abramson2024, WohlwendBoltz124, Watson2023}. Third, recent work by \cite{paulo2025sparseautoencoderstraineddata} shows that SAEs can learn different features when trained on the same data, suggesting our results may be sensitive to both initialization and our data sample of UniRef50. Fourth, many extracted features remain difficult to interpret, requiring extensive probing to identify biologically relevant ones.

% Additionally, our interventions on ESMFold were limited to manipulating single features and only on embeddings from individual layers, rather than exploring combinations of features or cross-layer interactions. Our structural steering experiments focused primarily on surface accessibility, leaving many other potential structural properties unexplored and the observed hydrophobicity effects could potentially be achieved through simpler approaches like steering small PLMs for direct sequence modifications or supervised linear probes.  The Matryoshka architecture, while effective, requires careful tuning of group sizes and may not scale efficiently to even larger models. Furthermore, our Swiss-Prot concept evaluation relies on existing annotations, potentially missing novel biological features that aren't yet documented. Finally, while we demonstrate preservation of structural information through ablation studies, we have not fully characterized how feature interactions in the SAE might affect ESMFold's folding mechanism.

\subsection{Future Work}

\textbf{Connections to Geometric Representations.} This work, while taking a significant step towards interpreting protein structure prediction, focuses primarily on learning linear representations of sequence information. Future work could establish formal connections between SAE sequence representations and equivariant representations of geometric data \citep{ThomasTFN18, geiger2022e3nneuclideanneuralnetworks, LeeEquifold22}, particularly investigating how the linear overcomplete basis learned by SAEs map to irreducible representations of geometric transformations in the context of protein structure prediction.

\textbf{Theoretical Analysis of Matryoshka SAEs.} Additionally, theoretical analysis drawing from ordered autoencoding \citep{rippel2014learningorderedrepresentationsnested, xu21anytime} and information bottleneck methods \citep{tishby2000informationbottleneckmethod} applied to protein structure prediction could improve our understanding of multi-scale feature learning in biological sequences. Such analysis may provide deeper insights into how hierarchical feature representations emerge and interact within the context of protein language models.


==> intro/intro_v1.tex <==
Protein structure prediction models have achieved remarkable success by leveraging vast amounts of sequence data \citep{Jumper2021, Lin2022.07.20.500902}. However, despite their impressive performance, we lack a clear understanding of how these models transform sequence information into structural predictions. Understanding these mechanisms would enable scientists to better diagnose model limitations and exert more precise control over structural predictions.

Recent investigations into these models have revealed key insights about their inner workings. Through careful analysis of model behavior, \citet{Ovc2024} demonstrated that protein language models predict structure primarily by memorizing and retrieving patterns of coevolving residues rather than learning fundamental biophysical principles. While this finding illuminates the broad strategy these models employ, it does not provide a complete picture of how specific model components contribute to structural predictions.

Mechanistic interpretability offers a complementary approach by directly analyzing the learned representations within these models. In particular, sparse autoencoders (SAEs) provide a promising unsupervised method for understanding model behavior by decomposing dense neural representations into a small set of human-interpretable features \citep{templeton2024scaling}. This approach has proven especially valuable for large language models, where complex behaviors often emerge from the interaction of many components.

SAEs have previously been trained on protein language models in the ESM2 series \citep{Simon2024.11.14.623630, Adams2025.02.06.636901}, identifying thousands of features which correspond to manually-annotated biological concepts and functional properties. However, the subject PLMs used in previous works were too small to enable interpretability on ESMFold, the structure prediction head on top of ESM2.

Our work bridges this gap by scaling SAE training to ESM2-3B, the base model for ESMFold, enabling the first mechanistic interpretability studies of protein structure prediction. We introduce Matryoshka SAEs, an architecture that organizes sparse features hierarchically, improving both model performance and human interpretability. Through comprehensive evaluations on both sequence-based annotations and structural predictions, we demonstrate that SAEs trained on ESM2-3B capture significantly more biological concepts than those trained on smaller models, validating the importance of analyzing more capable subject models.

Key Contributions:
\begin{enumerate}
    \item Train and evaluate SAEs on the largest PLM to date, ESM2-3B, enabling SAE interventions on ESMFold, a protein structure prediction model for the first time.
    \item Develop Matryoshka SAEs that organize features hierarchically in nested layers, allowing SAEs to learn high and low-level features.
    \item Demonstrate significant gains for ESM2-3B vs 8M on sequence and structure-based evaluations, highlighting the utility of using SAEs trained on a larger subject model.
    \item Present an initial steering case study on ESMFold where we increase hydrophobicity of the predicted structure without changing the input sequence.
\end{enumerate}

To enable the community to continue investigating, we will release our code and trained models open-source accompanied by a visualizer upon publication.

==> intro/intro_v2.tex <==
Machine learning-based protein structure prediction models have achieved remarkable success by leveraging vast amounts of sequence data \citep{Jumper2021, Lin2022.07.20.500902}, building on the success of previous sequence homology-based methods \citep{marks2011couplings, gremlin2013}. However, their nonlinear nature prevent easily understanding how sequence information informs structure prediction compared to previous statistical methods with simple linear priors.

Previous interpretability studies on transformer-based protein language models (PLMs) have demonstrated PLMs, despite only training on sequences, learn structural information. \citet{rao2021transformer} and \citet{vig2021bertologymeetsbiologyinterpreting} showed that the attention map learns to predict residue-residue contacts. \citet{Ovc2024} show PLMs predict structure primarily by memorizing and retrieving patterns of coevolving residues rather than learning fundamental biophysical principles. However, these works are limited to correlational analyses between model behaviors and biological patterns, failing to establish causal relationships between internal mechanisms and predictions.

Mechanistic interpretability through sparse autoencoders (SAEs) offers a promising direction for understanding these black box models by learning interpretable linear representations \citep{templeton2024scaling, gao2024scalingevaluatingsparseautoencoders}, similar to how earlier statistical methods successfully used linear priors to capture sequence-structure relationships. While modern PLMs achieve superior performance through complex nonlinear transformations, SAEs can potentially bridge this interpretability gap by decomposing these transformations into human interpretable features in a linear high-dimensional latent space. SAEs have previously been trained on protein language models in the ESM2 series \citep{Simon2024.11.14.623630, Adams2025.02.06.636901}, identifying thousands of features which correspond to manually-annotated biological concepts and functional properties. However, the subject PLMs used in previous works were too small to enable interpretability on ESMFold, the structure prediction head on top of ESM2.

Our work advances protein model interpretability in two key directions. First, we scale SAEs to ESM2-3B, the base model for ESMFold, enabling mechanistic interpretability of protein structure prediction for the first time. Second, we adapt Matryoshka SAEs \citep{nabeshima2024matryoshka, bussmann2024matryoshka} to PLMs, which learn features at multiple scales of detail. This hierarchical organization not only aligns with the multi-scale nature of protein structure but also improves feature disentanglement and interpretability compared to standard sparse autoencoders.

We structure the paper as follows:
\begin{enumerate}
    \item In Section 2, we present our methodological advances: scaling SAEs to ESM2-3B and adapting Matryoshka SAEs, a recently developed SAE architecture that learns hierarchically organized features.
    \item In Section 3, we validate our approach by demonstrating Matryoshka SAEs achieve comparable or better performance than L1 and TopK architectures on both language modeling and structure prediction tasks.
    \item In Section 4, we show the benefits of interpreting larger PLMs through ESM2-3B's superior performance on biological concept discovery and contact map prediction tasks.
    \item In Section 5, we demonstrate practical applications through an initial steering case study, showing how we can increase the solvent accessibility of a predicted structure while fixing the input sequence.
\end{enumerate}

To enable the community to extend our work and continue investigating, we will release our code and trained models open-source accompanied by a visualizer upon publication.

==> methods/background_v1.tex <==
\subsection{Setup} 
\textbf{Problem Statement.} 
For each token of a protein sequence, a transformer encoder-based PLM outputs an embedding \( x \in \mathbb{R}^{d} \) in each layer \( \ell \). A sparse autoencoder encodes the embedding  $x$  to a higher-dimensional latent representation $z \in \mathbb{R}^n$ where $d << n$ and decodes it as $\hat{x}$. The SAE is trained by minimizing the L2 reconstruction loss between the original embedding $x$ and its reconstruction $\hat{x}$, defined as $\mathcal{L} = \left\| x - \hat{x} \right\|^2_2$. 

To learn meaningful representations, sparsity constraints are imposed on the latent vector $z$. This sparsity can be achieved either through L1 regularization terms in the loss function or through specialized activation functions that directly restrict the number of non-zero elements. In practice, the number of active (non-zero) elements $K$ satisfies $K \ll d \ll n$, preventing degenerate solutions such as the identity map.

\textbf{Subject Models.} We train SAEs on the ESM2 series of PLMs \citep{Lin2022.07.20.500902}. We focus primarily on the 3 billion parameter model ESM2-3B which provides representations for ESMFold.

\textbf{Hyperparameters.} We train SAEs on layer 18 and 36 of ESM2-3B, the middle and last layer respectively. During training, we normalize our embeddings to have average unit L2 norm enabling hyperparameter transfer between layers. During inference, we unnormalize by scaling the biases following \citet{marks2024dictionary_learning}.

\textbf{Data.} We randomly selected 10M sequences from Uniref50, the training set of ESM2, constituting 2.5 billion tokens. See Appendix \ref{app:data_curation} for details.

==> tables/casp14_table.tex <==
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lcc}
    \toprule
    Comparison & BB RMSD (Å) \\
    \midrule
    Exp vs ESMFold & 9.679 \\
    Exp vs ESMFold w/ ESM2 Ablated & 16.027 \\
    Exp vs ESMFold w/ ESM2 L36 Only & 9.773 \\
    Exp vs SAE & 9.656 \\
    ESMFold vs SAE & 7.100 \\
    \bottomrule
\end{tabular}%
}
\caption{}
\label{tab:rmsd_comparison}

==> tables/model_comparison_sparsity.tex <==
\begin{table}[htbp]
  \centering
  \resizebox{0.9\linewidth}{!}{%
    \begin{tabular}{cccc}
      \toprule
      Model Arch & L0 & L1 Penalty & Loss Recovered (\%)  \\[0.5ex]
      
      \midrule
      Matryoshka  & 128 &  & 98.7  \\
      TopK  & 128 &  & 98.5 \\
      L1 Penalty & 116 & 0.015 & 95.5 \\
      \bottomrule
    \end{tabular}%
  }
  \caption{Your caption here.}
  \label{tab:3x4_table}
\end{table}

